Authoring image decompositions with generative models

We show how to extend traditional intrinsic image decompositions to incorporate further layers above albedo and shading. It is hard to obtain data to learn a multi-layer decomposition. Instead, we can learn to decompose an image into layers that are "like this" by authoring generative models for each layer using proxy examples that capture the Platonic ideal (Mondrian images for albedo; rendered 3D primitives for shading; material swatches for shading detail). Our method then generates image layers, one from each model, that explain the image. Our approach rests on innovation in generative models for images. We introduce a Convolutional Variational Auto Encoder (conv-VAE), a novel VAE architecture that can reconstruct high fidelity images. The approach is general, and does not require that layers admit a physical interpretation.

==> Decomposition.tex <==
\section{Decomposition}
Our decomposition models take the following general form.
We assume that the VAE decoder $D$ generally produces a high quality
image $D(z)$ when given a reasonable value of $z$.  We also assume
that we can bias the codes towards better values using a likelihood estimate
$P(z)$ learned on data (eg GMM).  Finally, we expect to include some image
priors $Q(D(z))$ such as parsimony, boundary conditions, or
total variation priors which capture phenomena which would be difficult
for a VAE decoder to learn.

\section{Shading Decomposition}
We start by decomposing shading into two channels, shading detail
and shading from effects on primatives.  This is a relatively
easy problem due to the significant differences in scale of the effects,
however, our results outperform simple baseline methods which attempt to
split up frequency responses.

In this case, we expect the intensity of
the lowest frequency of the shading detail to
be constant $\|S_d-mean(S_d)\|$, and the shading and shading detail to be
uncorrelated.  We also expect the estimated channels to sum to
the image $\|S_d + S_s = I\|$.

\section{Intrinsic Image Decomposition}
We decompose images into albedo and shading, as well as
albedo, shading, and shading detail.


